Safe Deep Reinforcement Learning by Verifying Task-Level Properties

Cost functions are commonly employed in Safe Deep Reinforcement Learning (DRL). However, the cost is typically encoded as an indicator function due to the difficulty of quantifying the risk of policy decisions in the state space. Such an encoding requires the agent to visit numerous unsafe states to learn a cost-value function to drive the learning process toward safety. Hence, increasing the number of unsafe interactions and decreasing sample efficiency. In this paper, we investigate an alternative approach that uses domain knowledge to quantify the risk in the proximity of such states by defining a violation metric. This metric is computed by verifying task-level properties, shaped as input-output conditions, and it is used as a penalty to bias the policy away from unsafe states without learning an additional value function. We investigate the benefits of using the violation metric in standard Safe DRL benchmarks and robotic mapless navigation tasks. The navigation experiments bridge the gap between Safe DRL and robotics, introducing a framework that allows rapid testing on real robots. Our experiments show that policies trained with the violation penalty achieve higher performance over Safe DRL baselines and significantly reduce the number of visited unsafe states.

==> Sections/old/old_intro.tex <==
\section{Experiments}
\label{sec:experiments}

First, we introduce a set of Turtlebot3-based safety mapless navigation tasks to enable rapid testing of policies in realistic contexts. Our environments rely on Unity \cite{unity} as it allows rapid prototyping, Gym compatibility \cite{Gym}, and interface with the \href{www.ros.org}{Robotic Operating System (ROS)}. Mapless navigation is a well-known problem in model-free DRL and prior Safe DRL literature
\cite{SafetyGym, AAAI_Sos, drl_navigation1, drl_navigation2}. While standard navigation planners use a map of the environment and exhaustive information from the sensors, DRL setups consider more challenging conditions, such as not having a map and relying only on sparse local sensing.
We use a similar encoding to prior work \cite{drl_navigation1, drl_navigation2, drl_navigation3, marche2020discrete, curriculum}: 11 sparse laser scans with a limited range and two values for the target relative position (i.e., distance and heading) as observations. Discrete actions encode angular and linear velocities to reduce training times while maintaining good navigation skills \cite{marche2020discrete}.\footnote{Our environments also support continuous actions and different domain randomization of the tasks and physical properties through the Unity editor.} At step $t$, the agent receives a reward:
\begin{equation}
    r_t = \begin{cases}
    1 \quad \hfill \text{if goal reached} \\
    \Delta(d_{t-1}, d_{t}) - \beta \quad \hfill \text{otherwise}\\
    %\begin{cases}
    %    0 \hfill~\text{if no collision or penalty }\\
    %    1 \quad \text{o.w.}
    %\end{cases}\\
    
    \end{cases}
\end{equation}
The agent thus obtains a dense reward given by the distance ($d$) difference ($\Delta$) from the goal in two consecutive steps, with a per-step $-\beta$ to incentive shorter paths. Each collision returns an additional signal that can be used to compute the desired penalty (e.g., cost, violation), enabling a straightforward application to different penalty-based objectives (as in Equation \ref{eq:penaltyobj}) or constraints.

We introduce four training and one testing environments with different obstacles, namely \textit{Fixed\_obs\_\{T, NT\}}, \textit{Dynamic\_obs\_\{T, NT\}}, and \textit{Evaluation\_NT} depicted in Figure \ref{fig:exp_envs}. Such a variety of conditions serve to provide different settings for evaluating Safe DRL algorithms in robotic navigation. The environments inherit several characteristics from known benchmarks such as SafetyGym \cite{SafetyGym} and differ from each other as the obstacles that can be \textit{Fixed} (parallelepiped-shaped static objects) or \textit{Dynamic} (cylindrical-shaped objects that move to random positions at a constant velocity). Moreover, obstacles can be \textit{Terminal} (T) if they end an episode upon collision, or \textit{Non-Terminal} (NT) if the agent can navigate through them.\footnote{Appendix 1 describes our environment in more detail.}
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/envs_new.png}
    \caption{Fixed, Dynamic, Evaluation tasks with different obstacles. Terminal obstacles (T) reset the environment upon collision. Non-terminal ones (NT) allow the robot to cross them, experiencing more unsafe states. The evaluation environment has fixed and dynamic non-terminal obstacles.}
    \label{fig:exp_envs}
\end{figure}

\begin{table*}[h]
    \centering
    \caption{Average \textit{violation} (\%), and computation time for properties $p_{\uparrow, \leftarrow, \rightarrow}$ calculated using ProVe\cite{prove}, and our approximation with 100, 1.000, and 10000 samples.}
    \label{tab:results:comparison}
    \begin{tabular}{lcccc}
      \toprule
      \bfseries Property & \bfseries ProVe & \bfseries Estimation 100 & \bfseries Estimation 1k & \bfseries Estimation 10k \\
      \midrule
      \textit{$p_{\uparrow}$} &  81.48 $\pm$ 1.2 & 81.0 $\pm$ 0.6 & 81.1 $\pm$ 0.8 & 81.17 $\pm$ 0.5 \\
       \textit{$p_{\leftarrow}$} & 73.9 $\pm$ 0.8  & 73.5 $\pm$ 0.2 & 73.63 $\pm$ 0.2 & 73.65 $\pm$ 0.3 \\
      \textit{$p_{\rightarrow}$} & 74.2 $\pm$ 0.3 & 73.6 $\pm$ 0.1 & 73.67 $\pm$ 0.1 &  73.68 $\pm$ 0.1 \\
      \midrule
      \textbf{Mean violation:} & \textbf{76.53} & 76.00 & 76.13 & \textbf{76.17} \\
      \midrule
      \textbf{Mean computation time:} & $\approx$\textbf{2m37s} & $\approx$\textbf{0.053s} & $\approx$ \textbf{0.056s} & $\approx$\textbf{0.060s} \\
      \bottomrule
    \end{tabular}
\end{table*}

\subsection{Properties for Mapless Navigation}\label{sec:design_prop}
Our hard-coded input-output conditions (properties) shape rational, safe behaviors for mapless navigation and are used to compute the approximate violation. Moreover, we consider an online generated property as described in Section \ref{sec:approx_vr}. A natural language description of the main hard-coded properties follows: 
\begin{itemize}
    \item $p_{\uparrow}$: \textit{There is an obstacle close in front $\Rightarrow$ Do not go forward}
    \item $p_{\leftarrow}$: \textit{There is an obstacle close to the left $\Rightarrow$ Do not turn left}
    \item $p_{\rightarrow}$: \textit{There is an obstacle close to the right $\Rightarrow$ Do not turn right}
\end{itemize}
Considering safety contexts, we assume having task-level knowledge to shape such properties, as discussed in our limitations. We use the maximum agent velocity to determine the size of the area around the (unsafe) states of interest (i.e., the $\pmb{\epsilon}$-area). For example, a formal definition for $p_{\uparrow}$ is:
\begin{equation*}
\begin{split}
    p_{\uparrow}:\; &x_0,\dots,x_4 \in [0, 1] \wedge x_5\in [0, 0.05]\wedge x_6,\dots,x_{10} \in [0, 1] \wedge x_{11},\\
    &x_{12}\in [-1, 1] \implies a \neq 4
\end{split}
\end{equation*}

where $x_0, \dots, x_{10}$ are the 11 lidar values, $x_{11}, x_{12}$ is the relative position of the goal (i.e., distance and heading), and action $a=4$ corresponds to a forward movement. 
Crucially, each input $x_i$ potentially considers a different interval to model the area of interest. Hence, $p_{\uparrow}$ checks the policy's decisions when there is an obstacle close to the front (i.e., $x_5\in [0, 0.05]$) under any possible target position ($x_{11}, x_{12} \in [-1, 1]$).\footnote{We measured that a minimum normalized distance of $0.05$ is required for the robot to turn at max speed and avoid obstacles in front.} The approximate violation computed over these properties thus contains information about a specific unsafe situation under a general goal configuration (i.e., $x_{11}, x_{12} \in [-1, 1]$).

To assess how good our approximate violation is over the provable one, we compare it with the violation computed by a FV framework \cite{prove}. In particular, both the formal violation and our approximate one are computed using the above properties and are averaged over the same ten models collected at random steps during the training. Table \ref{tab:results:comparison} shows the violation values for each property $p_{\uparrow, \leftarrow, \rightarrow}$ computed by ProVe \cite{prove}, and our approximation using 100, 1000, and 10000 samples. Crucially, our approximation shows an average $0.69\%$ error over the formal violation even when using only 100 samples. Such an error further decreases to $0.47\%$ by using 10000 samples. By exploiting parallelism and batch computation of modern Deep Learning Frameworks, the increase in computation time for the approximate violation with 100 or 10000 samples is comparable. Conversely, as discussed in Section 3.1, ProVe's average computation time is orders of magnitude higher with respect to our approach (i.e., 0.06 over 157 seconds). Our approximate methodology, however, does not formally guarantee the policy behaviors due to its sample-based nature. For this reason, the next section uses standard FV frameworks on the trained policies to show the provable violation results.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/exp_results_NT.png}
    \caption{The two rows show average success, cost, and violation in the (NT) environments for PPO, the cost and violation penalty versions PPO\_\{cost, violation\}, and LPPO. * indicates penalty-based algorithms.}
    \label{fig:exp_results}
\end{figure*}

\subsection{Empirical Evaluation}
Our evaluation aims at showing the following: 

\begin{itemize}
    \item The benefits of integrating reward and safety specifications into a single MDP.
    \item The advantages of using our violation over indicator cost functions. To assess our claims, we plot the following values averaged over the last 1000 steps: (i) success (i.e., the number of goals reached), (ii) cost, (iii) and the violation at different stages of the training.
\end{itemize}

Data are collected on an i7-9700k and consider the mean and standard deviation of ten independent runs \cite{colas2019hitchhikers}. We consider the cost and violation penalty objective (\ref{eq:penaltyobj}) in a value-based (Dueling Double Deep Q-Network (DuelDDQN) \cite{DuelDDQN}) and policy-based (PPO \cite{PPO}) baselines, referring to the resultant algorithms as DuelDDQN\_\{cost, violation\} and PPO\_\{cost, violation\}. We compare with Lagrangian PPO (LPPO) \cite{Lagrangian} as it is a widely adopted Constrained DRL baseline and achieves state-of-the-art performance in similar SafetyGym navigation-based tasks.\footnote{For a fair comparison, we set the cost threshold of LPPO to the average cost obtained by PPO\_cost. Appendix 4 details our hyper-parameters.} According to the literature, the value-based and policy-gradient baselines should achieve the highest rewards and costs (having no penalty information) \cite{SafetyGym}. Conversely, LPPO should show a significant trade-off between average cost and reward or fail at maintaining the cost threshold when set to low values \cite{IPO, SafetyGym, AAAI_Sos}. In contrast, we expect the penalty-based methods to achieve promising returns while significantly reducing the cost and the number of violations during the training. %We also aim to confirm the lack of local information on the cost signal. However, given the natural relationships between cost and violation, we note that cost-penalty algorithms should reduce the number of violations, failing to achieve the performance of violation-penalty approaches.

\textbf{Terminal Results.} Our results are shown in Appendix 2. We notice that the information carried by the violation results in a significant performance advantage, maintaining similar or higher successes over non-violation-based approaches. Moreover, the policy-based algorithms show superior performance over the value-based implementations.

\begin{table*}[t]
\centering
    \caption{Average formal violation for the models at convergence in NT environment. Our violation-based penalty algorithm is the safest overall, as a lower violation value translates into fewer collisions.}
    \label{fig:suppl_verification}
    \includegraphics[width=0.8\linewidth]{images/exp_verification_NT.png}
\end{table*}

\textbf{Non-Terminal Results.} Given the higher performance of policy-based algorithms, the following experiments omit value-based ones. The two rows of Figure \ref{fig:exp_results} show the results of (NT) tasks. As in the previous evaluation, PPO achieves a higher number of successes and a higher cost. In contrast, LPPO satisfies the constraint most of the time but achieves the lowest successes and does not learn effective navigation behaviors in \textit{Dynamic\_obs\_NT}, confirming the performance trade-off in complex scenarios \cite{SafetyGym, AAAI_Sos}. Moreover, PPO\_violation achieves better or comparable successes and cost values over PPO\_cost but significantly reduces the violations during the training. At convergence, PPO\_violation shows a $\approx2.2\%$ and $\approx4.6\%$ improvement over the cost counterparts, corresponding to 1320 and 2760 fewer unsafe policy decisions. In general, non-terminal tasks allow experiencing more unsafe situations in a trajectory, making the performance advantage in terms of safety of violation-based algorithms more evident. 

In addition, we use FV \cite{prove} on the trained models of NT environments to provably guarantee the number of unsafe policy decisions over our safety properties. 
Table \ref{fig:suppl_verification} shows the average violations of the main properties for the models at the convergence of each training seed, which confirms that policies trained with PPO\_violation achieve lower violations, i.e., perform fewer collisions. We note that FV frameworks typically return all the states where the policy violates the properties. Hence, it would be possible to design a shield to avoid unsafe behaviors at deployment. However, this is out of the scope of our work and is a direction for future work. Appendix 2 shows the same results for the T environments.

\textbf{Evaluation Results.} Table \ref{tab:exp_eval} reports average success, cost, and violation for the best model at convergence of each training seed in the evaluation task of Figure \ref{fig:exp_envs}. The evaluation in a previously unseen scenario is used to test the generalization skills of the trained policies. In our experiments, the violation-based algorithm confirms significant superior navigation skills, achieving more success while being safer than LPPO and the cost counterpart. 
\begin{table}[b]
\centering
    \caption{Performance of the best trained models in the testing environment \textit{Evaluation\_NT}.}
    \begin{tabular}{@{}lccc}
        \toprule
        & \multicolumn{1}{l}{Mean Success} & \multicolumn{1}{l}{Mean Cost} & \multicolumn{1}{l}{Mean Violation} \\ \midrule
        PPO & \textbf{10.0} $\pm$ 0.4 & 52.0 $\pm$ 4.8 & 63.7 $\pm$ 11.3 \\
        PPO\_cost & 6.4 $\pm$ 1.8 & 25.5 $\pm$ 8.3 & 29.2 $\pm$ 9.5 \\
        PPO\_violation & 7.7 $\pm$ 0.2 & \textbf{17.9} $\pm$ 1.2 & \textbf{18.8} $\pm$ 1.7 \\
        LPPO & 2.5 $\pm$ 0.3 & 18.2 $\pm$ 2.5  & 19.5 $\pm$ 0.9  \\
        \end{tabular}
    \label{tab:exp_eval}
\end{table}

\textbf{Real-Robot Testing. The core motivation for introducing our Safe DRL environments is the need for benchmarks that allow testing the policies directly on real robots. In contrast, Unity environments enable the transfer of policies trained in simulation on ROS-enabled platforms. 
Supplementary material contains a video with the real-world experiments of the policies trained in our environments, and Figure \ref{fig:exp_real} shows our actual setup with the Turtlebot3.

\begin{figure}[b]
    \centering
    \includegraphics[width=0.4\linewidth]{images/exp_real.jpg}
    \captionof{figure}{Overview of real-world experiments.}
\label{fig:exp_real}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/suppl_ablationprop.png}
    \caption{Average performance of penalty-based PPO using different pre-condition shapes: (i) fixed size (i.e., with a constant $\pmb\epsilon$), (ii) and one that considers the whole domain for the target's coordinates (i.e., different values for $\pmb\epsilon$. For example, $x_{11, 12} \in [-1, 1]$).}
    \label{fig:suppl_epsilonexp}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{images/suppl_nproperties.png}
    \caption{Mean size of $P'$ over the training for PPO\_violation with an online generated property (red), and with only the hard-coded properties (green).}
    \label{fig:suppl_nprop}
\end{figure}

\subsection{Additional Experiments}
We performed several additional experiments in the \textit{Fixed\_obs\_NT} task to highlight the impact of the different components presented in this paper: (i) using different sizes for the pre-conditions, (ii) the online property.\footnote{A regularization term can module the importance of the penalty over the training. We perform additional experiments with it in Appendix 3.} (iii) We show the results of our violation-based penalty method in standard safe locomotion benchmarks to further confirm the performance improvement of the proposed approach.

\textbf{Different Sizes for Pre-Conditions.} Figure \ref{fig:suppl_epsilonexp} shows the results of two PPO\_violation versions: one that uses a constant $\pmb{\epsilon}$ for the size of the pre-conditions, and one that has different $\pmb{\epsilon}$ values for each input. The latter considers all the possible target positions as in previous experiments. As detailed in Section \ref{sec:design_prop}, using wider ranges for the inputs that shape environment configurations allow the violation to contain details about the unsafe behavior in general target initialization, resulting in higher performance. Crucially, the PPO\_violation with a constant $\pmb{\epsilon}$ also returns better performance over PPO\_cost, confirming the importance of having locally-aware information in the penalty value. This is particularly important as it may not be possible to shape detailed pre-conditions in setups where accurate task-level knowledge is lacking. 

\textbf{Online Property.}
As detailed in Section 3.1, we generate an additional property upon experiencing an unsafe state $s$ because it is not uncommon to experience an unsafe transition not included in the pre-conditions (due to the limitation of hard-coding properties). Figure \ref{fig:suppl_nprop} shows the size of the set $P'$ during the training for PPO\_violation under two implementations. The first adds an online-generated property, and the second one uses only the hard-coded properties. Results for the latter show an average size of $P'$ $< 1$, confirming our hypothesis and the limitations of the properties' design of Section \ref{sec:limitations}. In contrast, the generated property implementation ensures having at least one input-output mapping for each unsafe state. This allows the violation to correctly shapes information about undesired situations, which biases the policy toward safer regions. Moreover, the growth in the size of $P'$ over the training indicates that the policy experiences unsafe states in rare corner cases captured by the intersection of multiple properties (i.e., some complex situations require not choosing more than one action to avoid collisions).

\textbf{Standard Safe DRL Tasks.}
We performed additional experiments in the standard Safe-AntCircle, and Safe-DroneRun, to consider a wider variety of simulated robots, tasks, and safety specifications.
Our goal is to confirm further our framework's results and the benefits of using the violation as a penalty in different domains known in the literature.\footnote{ We refer to the original works for more details about the environments \cite{CPO}, \url{github.com/SvenGronauer/Bullet-Safety-Gym}}
In more detail, we consider the same hyperparameters of our navigation experiments. Moreover, given the challenges of hand-writing properties for legged robots and drones, we rely on the online generated property only, considering a fixed $\epsilon$-area of size $0.05$ where we want to avoid a similar action that led to the unsafe state, up to decimal precision. 
The following results consider the average reward, cost, and violation collected over ten runs with different random seeds.

Figure \ref{fig:appendix_safetybullet} shows the results of Safe-AntCircle on the first row and Safe-DroneRun on the second. In contrast to previous results, in Safe-AntCircle, LPPO learns good behaviors while maintaining a low cost threshold set to 1. Nonetheless, the violation-based PPO maintains the best trade-off between reward and cost. Safe-DroneRun's results confirm the behavior of previous experiments (we omitted the PPO results to maintain the plot scale for better visualization), where LPPO struggles to keep the cost threshold set to 20 and results in lower performance compared to the penalty-based approaches.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/exp_additional_results.png}
    \caption{Average reward, cost, and violation in Safe-AntCircle and Safe-DroneRun for PPO, PPO\_\{cost, violation\}, LPPO. * indicates penalty-based algorithms.}
\label{fig:appendix_safetybullet}
\end{figure*}


==> Sections/old/old_intro_v2.tex <==
\section{Introduction}

Model-free Safe Deep Reinforcement Learning (DRL) approaches typically foster safety by maximizing a reward function while limiting the accumulation of costs caused by unsafe interactions \cite{Garcia2015}. However, defining informative cost functions has the same issues as designing rewards \cite{DiversityExpl} due to the difficulty of quantifying the risk in the proximity of unsafe states. For this reason, recent approaches usually rely on indicator functions, where a positive value deems a state as unsafe \cite{IPO, LagrangianBehavior}. In more detail, the cost refers to a state-action pair $(s, a)$ and is backed up to propagate safety information and estimate a cost-value function. Such a cost-value function then drives the learning process towards safety using penalties \cite{Garcia2015, RCPO}, cumulative constraints, or instantaneous ones \cite{Lagrangian, ConstrainedDRL}. However, as discussed by recent work \cite{DeepPG}, the learned value functions in state-of-the-art DRL algorithms have poor estimates and end up in local optima, limiting their efficacy for fostering safety. In addition, the sparse nature of indicator functions further exacerbates such an issue as the agent has to visit the unsafe states to collect the sparse feedback and learn good estimates. These issues are crucial in a safety context where we aim to improve sample efficiency to minimize the number of visited unsafe states. To this end, we note that typical cost functions do not consider areas around $s$ where it could be risky to perform the same action that led to deeming $s$ unsafe. For these reasons, we argue that cost functions are not \textit{locally-aware} as they lack using explicit task-level information about possible unsafe surroundings of a state, which is typically available in scenarios with safety requirements.

\begin{figure}[b]
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.7\linewidth]{images/intro_overall.png}
    \vspace{-0.1cm}
    \caption{We analyze the advantages of replacing indicator cost function (left) with checking the policy decisions in the surrounding $\epsilon$ of an unsafe state (right).}
    \label{fig:visual_example}
    \vspace{-0.3cm}
\end{figure}

As a realistic example, consider a navigation scenario where a policy chooses the robot's velocity given its current position. In such a context, prior Safe DRL methods \cite{IPO, Lagrangian, SafetyGym, Lyapunov, Lyapunov2} would trigger a positive cost in case of a collision in a specific state $s$, as depicted in Figure \ref{fig:visual_example} on the left. However, these approaches typically need to perform similar unsafe interactions in states around $s$ in order to learn an effective cost function to drive the learning process toward safety.
In contrast, we argue that it is possible to exploit high-level system specifications without having an explicit model (e.g., robots' maximum velocity, its dimension) to define an area around the unsafe state $s$ where performing the same action $a$ that led to collision would result in another similar risky interaction. Following this idea, we can avoid to explore such an \textit{unsafe} area to learn a cost-value function, and compute a risk value based on the current policy's decisions. Figure \ref{fig:visual_example} on the right depicts this scenario, where performing the previous action in the green area of size $\epsilon$ around $s$ would lead to other collisions. The idea is thus to replace indicator cost functions on state-action pairs and the learning of cost-value functions by quantifying the situations where the policy chooses $a$ in the hazardous area to provide more information about unsafe behaviors in the learning process. To this end, we require shaping the (unsafe) state-action mappings following known safety specifications and additional forward steps to check the policy against those mappings. Hence, significantly improving sample efficiency and limiting the number of visited unsafe states as we do not have to perform unsafe interactions to learn a cost-value function.

In this direction, we propose to rely on a \textit{violation} metric that uses task-level specifications to quantify how safe policy decisions are around $s$. We investigate the use of the violation as a penalty to discourage unsafe decisions \cite{RewardEngineering, Reward, RewardShaping}. 
Following recent literature \cite{Verification}, it is possible to encode whether a deterministic policy chooses specific actions (\textit{outputs}) in a subspace of the state space (\textit{inputs}) as an input-output conditional statement, commonly referred to as task-level \textit{properties} (i.e., the state-action mappings). Formal Verification (FV) approaches for Deep Neural Networks (DNNs) can then be used to formally check the inputs where the policy violates such properties \cite{Neurify}. Specifically, by using the violation metric introduced in \cite{prove}, it is possible to provably quantify how well a policy respects the properties, overcoming the issues of commonly used indicator cost functions. As such, we consider the violation to be a locally-aware cost function. However, DNN's verification has two main issues as (i) it is a \textit{NP-Complete} problem \cite{reluplex} and it is thus intractable to compute the formal violation value on continuous state spaces at training time to foster safety without a prohibitive overhead. (ii) The state-action mappings are typically hand-designed, which could be unfeasible in tasks with complex or unknown specifications. 

Against this background, we make the following contributions to the state-of-the-art: 
\begin{itemize}
    \item To address (i), we propose to substitute the FV framework with a sample-based approach that approximate the violation metric with computationally inexpensive forward propagations of the DNN on a limited number of states. Such an approximation empirically achieves a negligible error over the value computed with FV, requiring a fraction of the computation time.
    \item To address (ii), we investigate the benefits of generating a state-action mapping when performing an unsafe interaction during the training (i.e., using a fixed-size area around the visited unsafe state, and the action that led to the interaction). 
    \item We show the significant advantages of using our approximate violation as a penalty in existing DRL algorithms. Moreover, we employ a prior FV framework \cite{prove} on the trained policies to prove that our approach allows learning safer behaviors (i.e., results in a lower violation).
\end{itemize}

\noindent Our empirical evaluation shows that a penalty-based objective defined with the violation metric drastically reduces unsafe behaviors (measured in terms of cost and violation values) while preserving good returns. To this end, we introduce a set of Unity \cite{unity} robotic mapless navigation tasks \cite{drl_navigation1, drl_navigation2, drl_navigation3} based on the \href{www.turtlebot.com}{Turtlebot3} platforms. In contrast to Safe DRL benchmarks (e.g., SafetyGym \cite{SafetyGym} and SafeMuJoCo \cite{IPO}), the proposed scenarios allow transferring policies directly on the robot exploiting \href{www.github.com/Unity-Technologies/Unity-Robotics-Hub}{Unity Robotics} which is a key point to foster the development of Safe DRL approaches in realistic applications. We also confirm the superior performance of violation-based approaches in standard SafeMuJoCo scenarios. In all scenarios, we compare with unconstrained DRL baselines augmented with a cost penalty \citep{DuelDDQN, PPO}, and constrained DRL \cite{Lagrangian}. 
Empirical evidence confirms the lack of information provided by indicator cost functions, as cost-based algorithms have higher costs and higher violations. In contrast, our violation-based implementations obtain the lowest cost and violation during and after training, confirming the benefits of the violation metric to foster safety.\footnote{The environments, the code of the experiments, and the real robot experiments are available in the supplementary material.}


